Injecting Numerical Reasoning Skills into Language Models

Large pre-trained language models (LMs) are known to encode substantial amounts of linguistic information. However, high-level reasoning skills, such as numerical reasoning, are difficult to learn from a language-modeling objective only. Consequently, existing models for numerical reasoning have used specialized architectures with limited flexibility. In this work, we show that numerical reasoning is amenable to automatic data generation, and thus one can inject this skill into pre-trained LMs, by generating large amounts of data, and training in a multi-task setup. We show that pre-training our model, GenBERT, on this data, dramatically improves performance on DROP (49.3 $\rightarrow$ 72.3 F1), reaching performance that matches state-of-the-art models of comparable size, while using a simple and general-purpose encoder-decoder architecture. Moreover, GenBERT generalizes well to math word problem datasets, while maintaining high performance on standard RC tasks. Our approach provides a general recipe for injecting skills into large pre-trained LMs, whenever the skill is amenable to automatic data augmentation.

==> 01_introduction_old.tex <==
\section{Introduction}



\jb{structure of intro should be improved: (a) numerical reasoning is a core thing and DROP tests that (b) Recent neural models that are BERT-based very quickly reached high accuracy. (c) In this work we ask whether these models learn to do this in a generalizable manner. We first (d) develop automatic method for generating adversarial examples and show that in many cases current models are not robust (e) We propose new models for improving the robustness of these models by pre-training (f) new model architectyures (g) Empirically we show on DROP that ...}


Numerical reasoning is a core capability of humans essential for understanding natural language text. 
The recent Discrete Reasoning Over Passages (DROP) \cite{dua2019drop} dataset challenges reading comprehension models with questions involving numerical reasoning over numbers and dates.
In a short amount of time after its initial release, substantial progress has been reported on DROP, with BERT-extended neural models achieving state-of-the-art performance \cite{hu2019multi, andor2019giving}, hinting to the existence of numerical representations in pre-trained embeddings \jb{cite numbers paper}.
But do these modesl truly learn to perform quantitative reasoning in a generalizable manner?

Models trained on DROP learn to choose an arithmetic expression over numerical text pieces from the paragraph that evaluates to the correct answer. Therefore, interpreting the numerical value of text pieces and performing basic mathematical operations are learned implicitly.
\mg{Maybe we should also include something about the complexity of current models compared to generative neural models as part of the motivation.}
As a result, models trained on DROP are extremely sensitive to the data distribution of numbers and arithmetic expressions, leading to easy-to-break mathematical skills and poor generalization to out of distribution examples.

In this work, we systematically demonstrate the brittleness of current models for numerical reasoning and propose methods for making these models more robust, through adversarial data augmentation and better numerical text representations.
\mg{More details on what we're doing and showing in this work...}


==> 06_analysis.tex <==
\section{Testing Model Robustness and Generalization}
\label{section:model_performance_analysis}

A model that can numerically reason over text, should be able to perform discrete operations such as locating entities from the question in the given context, extracting quantities and dates related to them, and aggregating results through operations such as maximum and minimum, count, and addition and subtraction.
For example, to answer the first question (Q1) in Table~\ref{table:drop_example}, the model needs to extract the founding years of the two galleries mentioned in the question (i.e. 2007 and 2008), and then calculate the difference $2008-2007=1$ to reach the final answer.

To test model robustness and generalization, we use data augmentation to generate challenge examples targeting specific skills (Section~\ref{section:data_augmentators}). We augment the development set of DROP to create a challenge dataset (Section~\ref{section:augmented_drop}), and analyze the performance of \genbert{} (Section~\ref{section:model_performance_augmented_drop}).

\subsection{Data Augmentators}
\label{section:data_augmentators}
To test the reasoning skills of a model, we implement \textit{data augmentators}, i.e. methods for generating examples based on examples from the original dataset. We build augmentators of three types (listed in Table~\ref{table:data_augmentators}):

\paragraph{Shallow augmentators}
A model with robust reasoning skills would not rely on shallow matching patterns between the question and the context.
Shallow augmentators target such behaviors by inducing local perturbations in the data. 
The \texttt{order-swap} augmentator swaps the order of two objects \nl{X and Y} to \nl{Y and X}, and the \texttt{patch} augmentator concatenates an entity from the question and a number to the end of the passage.
A model that answers merely based on local information in the passage will be distracted by these perturbations. \mg{cite similar papers about SQuAD?}

Considering the example in Table~\ref{table:drop_example} (Q1), if a model successfully answers the given question, but fails to answer \nl{When was Art Euphorie founded?}, then it reaches the original answer without performing the entire reasoning process.
Therefore, querying the model on intermediate steps of the reasoning process, could indicate whether the model exploits artificial artifacts in the data. Intermediate augmentators take multi-step reasoning questions and generate new questions on intermediate steps. The last question on Art Euphorie, for instance, would have been created by the augmentator \texttt{HowManyAfter}.

\paragraph{Modifying augmentators}
The last type of augmentators leverages patterns in the data to modify the reasoning process, where each modifying augmentator targets a specific skill. For example, \texttt{antonym} tests the model's understanding of comparatives by switching comparative words with their antonyms.
The \texttt{range} augmentator


\subsection{DROP Augmented Data}
\label{section:augmented_drop}

We generate a challenge dataset by running the data augmentators described in Section~\ref{section:data_augmentators} and in Table~\ref{table:data_augmentators} on the development set of DROP.
\mg{specify the subsets - superlatives, comparatives, etc.}
For the shallow augmentators \texttt{PatchStart} and \texttt{PatchEnd} we randomly choose $63$ as the number to patch to passages. \mg{probably we should choose the number in a more elegant way? or maybe report a few numbers?}
The antonyms of comparative words were obtained using the Spacy WordNet annotator.\footnote{\texttt{https://spacy.io/universe/project/spacy-wordnet/}}
We also compose the two augmentators \texttt{CompAntonym} and \texttt{CompOrder} to create a new augmentator \texttt{CompAntonymOrder} for comparison questions.
\mg{We can provide much more details here on the augmentators, but I'm wondering if this is necessary given that the code will be published.}

% We manually analyzed 50 random generated examples from each augmentator to verify the resulting examples are answerable as expected and that the generated text is grammatically and semantically correct. \mg{need to do that...}

Statistics on the resulting challenge dataset are provided in Table~\ref{table:adversarial_data_stats}. Overall, most of the generated examples originate from the shallow augmentators, which assume very few or no properties of the data.

Our code for data augmentators and the generated examples are publicly available at: \texttt{anonymized}. 


\subsection{Model Performance on Augmented Data}
\label{section:model_performance_augmented_drop}
Performance breakdown by augmentator in Figure~\ref{figure:performance_by_augmentator} 


\begin{figure}
    \centering
    \includegraphics[scale=0.36]{figures/drop_dev_orig_vs_augmented_performance.pdf}
    \caption{Performance breakdown on DROP development set by augmentator.}
    \label{figure:performance_by_augmentator}
\end{figure}


\begin{table*}[t]
\begin{center}
\footnotesize
\begin{tabular}{l|p{4.0cm}|p{8.0cm}}
\multicolumn{1}{c}{\bf Augmentator} & \multicolumn{1}{c}{\bf Description} & \multicolumn{1}{c}{\bf Example} \\ \toprule
\multicolumn{3}{c}{\bf Robustness} \\ \hline
\multirow{3}{*}{\texttt{patch}} & \multirow{3}{4.0cm}{Patching an question entity and a number at the end of passages} & $q$: How many new Peso notes were presented in 1944? \\
 & & $p$: ...inflation experienced in January 1944. \\
 & & $p^*$: ...inflation experienced in January 1944. \textbf{Peso 63.} \\\hline
\multirow{2}{*}{\texttt{order-swap}} & \multirow{2}{4.0cm}{Replacing the order of objects in comparison questions} & $q$: Which ancestral group is smaller: \textbf{English or Irish}? \\
 & & $q^*$: Which ancestral group is smaller: \textbf{Irish or English}? \\\hline
 
\multicolumn{3}{c}{\bf Generalization} \\ \hline
\multirow{5}{*}{\texttt{selection}} & \multirow{5}{4.0cm}{Asking about the larger group in questions about the difference of two quantities} & $q$: How many \textbf{more} Democratic voters are there \textbf{than Republican}? \\
 & & $a$: 4,482 \\
 & & $q^*$: How many Democratic voters are there? \\
 & & $a^*$: 11,959 \\\hline

\multirow{6}{*}{\texttt{antonym}} & \multirow{6}{4.0cm}{Replacing the comparative with its antonym in comparison questions} & $q$: Which was \textbf{higher}, the homeowner vacancy rate or rental vacancy rate? \\
 & & $a$: rental vacancy rate \\
 & & $q^*$: Which was \textbf{lower}, the homeowner vacancy rate or rental vacancy rate? \\
 & & $a^*$: the homeowner vacancy rate \\\hline
\multirow{5}{*}{\texttt{ratio-swap}} & \multirow{5}{4.0cm}{Swapping the ratio of numbers correlated to compared objects in comparison questions} & $q$: Which group in Bahrain is larger: Indians or Bangladeshis? \\
 & & $p$: ...roughly 290,000 Indians, \textbf{125,000} Bangladeshis,... \\
 & & $a$: Indians \\
 & & $p^*$: ...roughly 290,000 Indians, \textbf{455,000} Bangladeshis,... \\
 & & $a^*$: Bangladeshis \\\hline
\multirow{5}{*}{\texttt{diff-to-sum}} & \multirow{5}{4.0cm}{Asking about the sum rather than the difference in questions about the difference of two numbers} & $q$: How many \textbf{more} masjids are there \textbf{compared to} Buddhist temples? \\
 & & $a$: 5 \\
 & & $q^*$: How many masjids \textbf{and} Buddhist temples are there? \\
 & & $a^*$: 73 \\\hline
 \multirow{2}{*}{\texttt{range}} & \multirow{2}{4.0cm}{Modifying the number range in the passage by adding / multiplying by a constant.} & $p$: \mg{example}... \\
 & & $p^*$: ... \\\hline
\end{tabular}
\end{center}
\caption{Data augmentators.}
\label{table:data_augmentators}
\end{table*}





==> 06_analysis_old.tex <==
\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{p{7.0cm}}
\toprule
\textbf{Passage}: \textit{Taunton has four art galleries... \textbf{\textcolor{NavyBlue}{Hughes/Donahue Gallery}} founded in \textbf{\textcolor{Orange}{2007}}, a local community gallery serving local Taunton artists... \textbf{\textcolor{NavyBlue}{Art Euphoric}} founded in \textbf{\textcolor{Orange}{2008}} has both visual and craft exhibits and sales...} \\ \hline
\textbf{Question}: \textit{How many \textbf{\textcolor{Orange}{years}} \textbf{\textcolor{Green}{after}} founding of \textbf{\textcolor{NavyBlue}{Hughes/Donahue Gallery}} was \textbf{\textcolor{NavyBlue}{Art Euphoric}} founded?} \\ \hline
\textbf{Answer}: 1 \\
\mg{Here we'll have adversarial example(s), maybe also the reasoning process (entity selection, number extraction, aggregation) leading to the final answer.}
% return year of the  founding of  the Hughes/Donahue Gallery ;return year when  Art Euphoric was  founded ;return the  difference of #2 and  #1
\\ \toprule
\end{tabular}
\end{center}
\caption{Example from DROP development set.}
\label{table:discrete_ops_example}
\end{table}


\section{Performance Analysis With Data Augmentators}
\label{section:model_performance_analysis}
\mg{! this entire section should be updated !}

A model that can numerically reason over text, should be able to perform discrete operations such as locating entities from the question in the given context, extracting quantities and dates related to them, and aggregating results through operations such as maximum and minimum, count, and addition and subtraction.
For example, to answer the question in Table~\ref{table:discrete_ops_example}, the model needs to extract the founding years of the two galleries mentioned in the question (i.e. 2007 and 2008), and then calculate the difference $2008-2007=1$ to obtain the final answer.

% To demonstrate the brittleness of current models, we start by analyzing their performance with respect to different properties of the data, while highlighting several unexpected behaviors observed through manual interactive queries (Section~\ref{section:performance_breakdown}).
% In addition, 
To systematically test the numerical reasoning skills of a model, we introduce three types of methods for generating adversarial examples, which we term \textit{adversarial augmentators} (Section~\ref{section:adversarial_augmentators}). We run our augmentators on DROP to create a challenge dataset (Section~\ref{section:adversarial_data_generation}), and analyze the performance of current state-of-the-art models on DROP (Section~\ref{section:model_performance_adversarial_data}).

\subsection{Data Augmentators}
\label{section:adversarial_augmentators}
To test the numerical reasoning skills of a model, we implement \textit{data augmentators}, i.e. methods for generating adversarial examples based on examples from the original dataset. We consider three types of augmentators (listed in Table~\ref{table:data_augmentators}):

\paragraph{Shallow augmentators}
We would expect that a model with robust reasoning skills would not rely on shallow surface matching patterns between the question and the context. 
Shallow augmentators target such behaviors by inducing local perturbations in the data. For example, \texttt{CompOrder} swaps the order of two objects \nl{X and Y} to \nl{Y and X}, and \texttt{PatchStart} simply concatenate a number to the beginning of the passage.
A model that answers merely based on local information in the passage, will be distracted by these perturbations. \mg{cite similar papers about SQuAD?}

\paragraph{Intermediate augmentators}
Considering the example in Table~\ref{table:discrete_ops_example}, if a model successfully answers the given question, but fails to answer \nl{When was Art Euphorie founded?}, then it reaches the original answer without performing the entire reasoning process.
Therefore, querying the model on intermediate steps of the reasoning process, could indicate whether the model exploits artificial artifacts in the data. Intermediate augmentators take multi-step reasoning questions and generate new questions on intermediate steps. The last question on Art Euphorie, for instance, would have been created by the augmentator \texttt{HowManyAfter}.

\paragraph{Modifying augmentators}
The last type of augmentators leverages patterns in the data to modify the reasoning process, where each modifying augmentator targets a specific skill. For example, \texttt{CompAntonym} tests the model's understanding of comparatives by switching comparative words with their antonyms. Similarly, \texttt{ComplPercent} targets understanding of percentages by modifying questions about the percentage of a group to be on the complementary group.


\subsection{DROP Augmented Data}
\label{section:adversarial_data_generation}

We generate a challenge dataset by running the adversarial augmentators described in Section~\ref{section:adversarial_augmentators} and in Table~\ref{table:data_augmentators} on DROP.
For the shallow augmentators \texttt{PatchStart} and \texttt{PatchEnd} we randomly choose $63$ as the number to patch to passages. \mg{probably we should choose the number in a more elegant way? or maybe report a few numbers?}
The antonyms of comparative words were obtained using the Spacy WordNet annotator.\footnote{\url{https://spacy.io/universe/project/spacy-wordnet/}}
We also compose the two augmentators \texttt{CompAntonym} and \texttt{CompOrder} to create a new augmentator \texttt{CompAntonymOrder} for comparison questions.
\mg{We can provide much more details here on the augmentators, but I'm wondering if this is necessary given that the code will be published.}

We manually analyzed 50 random generated examples from each augmentator to verify the resulting examples are answerable as expected and that the generated text is grammatically and semantically correct. \mg{need to do that...}

Statistics on the resulting challenge dataset are provided in Table~\ref{table:adversarial_data_stats}. Overall, most of the generated examples originate from the shallow augmentators, which assume very few or no properties of the data.

Our code for adversarial augmentators as well as the generated adversarial dataset are publicly available at: \url{anonymized}. 


\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{l|c|c}
        \bf Augmentator & \bf \# train & \bf \# dev \\ \hline
        \texttt{ListOrder} & 7,233 & 2,102 \\
        \texttt{PatchStart} & 77,409 & 9,536 \\
        \texttt{PatchEnd} & 43,233 & 5,089 \\
        \texttt{CompOrder} & 3,931 & 786 \\ \hline
        \texttt{HowManyMoreMax} & 1,534 & 334 \\
        \texttt{HowManyLonger} & 425 & 24 \\
        \texttt{HowManyAfter} & 293 & 35 \\ \hline
        \texttt{CompAntonym} & 3,341 & 693 \\
        \texttt{CompRatio} & 198 & 74 \\
        \texttt{ComplPercent} & 2,091 & 687 \\
        \texttt{HowManyMoreSum} & 631 & 192 \\ \hline 
        \texttt{CompAntonymOrder} & 3,341 & 693 \\ \hline
        \bf Total & 143,660 & 20,240 \\
    \end{tabular}
    \caption{Statistics on the adversarial dataset generated by running our augmentators on the train and development sets of DROP.}
    \label{table:adversarial_data_stats}
\end{table}


\subsection{Model Performance on Augmented Data}
\label{section:model_performance_adversarial_data}
\begin{itemize}
    \item NABERT+ performance breakdown by augmentator, after training on the original vs. augmented train set: Table~\ref{table:model_performance_adversarial}. Showing that training on the augmented data improves model robustness (performance on the adversarial dev data).
    \item Add a breakdown by domain (NFL/History)
    \item Add results for SOTA model by Google when their code is available
    \item Add results for MTMSN/NAQANet?
\end{itemize}


\begin{table*}[t]
    \footnotesize
    \centering
    \begin{tabular}{l|lccc}
        \bf Augmentator & \bf Train set & \bf EM orig. & \bf EM adv. & \bf diff. \\ \toprule
        \multirow{2}{*}{\texttt{ListOrder}} & original & 72.31 & 72.45 & +0.14 \\
         & augmented & 73.07 & 72.36 & -0.71 \\ \hline 
        \multirow{2}{*}{\texttt{PatchStart}} & original & 63.01 & 61.89 & -1.12 \\
        & augmented & 63.08 & 63.34 & +0.26 \\ \hline 
        \multirow{2}{*}{\texttt{PatchEnd}} & original & 60.96 & 55.9 & -5.06 \\
        & augmented & 60.82 & 61.05 & +0.23 \\ \hline 
        \multirow{2}{*}{\texttt{CompOrder}} & original & 77.86 & 69.85 & -8.01 \\
        & augmented & 81.42 & 80.28 & -1.14 \\ \toprule
        \multirow{2}{*}{\texttt{HowManyMoreMax}} & original & 88.92 & 80.54 & -8.38 \\
        & augmented & 88.62 & 89.82 & +1.2 \\ \hline 
        \multirow{2}{*}{\texttt{HowManyLonger}} & original & 87.5 & 91.67 & +4.17 \\
        & augmented & 91.67 & 87.5 & -4.17 \\ \hline 
        \multirow{2}{*}{\texttt{HowManyAfter}} & original & 74.29 & 71.43 & -2.86 \\
        & augmented & 82.86 & 80.0 & -2.86 \\ \toprule
        \multirow{2}{*}{\texttt{CompAntonym}} & original & 80.81 & 73.45 & -7.36 \\
        & augmented & 84.27 & 79.37 & -4.9 \\ \hline 
        \multirow{2}{*}{\texttt{CompRatio}} & original & 90.54 & 12.16 & -78.38 \\
        & augmented & 90.54 & 52.70 & -37.84 \\ \hline 
        \multirow{2}{*}{\texttt{ComplPercent}} & original & 86.32 & 62.01 & -24.31 \\
        & augmented & 85.44 & 86.90 & 1.46 \\ \hline 
        \multirow{2}{*}{\texttt{HowManyMoreSum}} & original & 98.96 & 92.71 & -6.25 \\
        & augmented & 96.88 & 93.75 & -3.13 \\ \toprule
        \multirow{2}{*}{\texttt{CompAntonymOrder}} & original & 80.81 & 66.67 & -14.14 \\
        & augmented & 84.27 & 79.37 & -4.9 \\ \toprule
        % \multirow{2}{*}{\bf Average} & original & 63.01 & 62.83 & -0.18 \\
        % & augmented & 63.08  & 66.95 & +3.87 \\
    \end{tabular}
    \caption{NABERT+ performance on the original and adversarial development sets of DROP, after training on the original and augmented train set of DROP. \mg{should add a graph to show these results.}}
    \label{table:model_performance_adversarial}
\end{table*}

\begin{table*}[t]
\begin{center}
\footnotesize
\begin{tabular}{l|p{4.0cm}|p{8.0cm}}
\multicolumn{1}{c}{\bf Augmentator} & \multicolumn{1}{c}{\bf Description} & \multicolumn{1}{c}{\bf Example} \\ \toprule
\multicolumn{3}{c}{\bf Shallow Augmentators} \\ \hline
\multirow{6}{*}{\texttt{ListOrder}} & \multirow{6}{4.0cm}{Permuting list elements in passages} & $p$: ...the population was spread out with 25.00\% under the age of 18, 17.10\% from 18 to 24, 25.70\% from 25 to 44, 19.30\% from 45 to 64, and 12.90\% who were 65 years of age or older... \\
 & & $p^*$: ...the population was spread out with 25.00\% under the age of 18, 19.30\% from 45 to 64, 25.70\% from 25 to 44, 17.10\% from 18 to 24, and 12.90\% who were 65 years of age or older... \\\hline
\multirow{2}{*}{\texttt{PatchStart}} & \multirow{2}{4.0cm}{Patching a number at the beginning of passages} & $p$: As of 2000, there were... \\
 & & $p^*$: \textbf{63.} As of 2000, there were... \\\hline
\multirow{3}{*}{\texttt{PatchEnd}} & \multirow{3}{4.0cm}{Patching an question entity and a number at the end of passages} & $q$: How many new Peso notes were presented in 1944? \\
 & & $p$: ...inflation experienced in January 1944. \\
 & & $p^*$: ...inflation experienced in January 1944. \textbf{Peso 63.} \\\hline
\multirow{2}{*}{\texttt{CompOrder}} & \multirow{2}{4.0cm}{Replacing the order of objects in comparison questions} & $q$: Which ancestral group is smaller: \textbf{English or Irish}? \\
 & & $q^*$: Which ancestral group is smaller: \textbf{Irish or English}? \\\hline
 
\multicolumn{3}{c}{\bf Intermediate Augmentators} \\ \hline
\multirow{5}{*}{\texttt{HowManyMoreMax}} & \multirow{5}{4.0cm}{Asking about the larger group in questions about the difference of two quantities} & $q$: How many \textbf{more} Democratic voters are there \textbf{than Republican}? \\
 & & $a$: 4,482 \\
 & & $q^*$: How many Democratic voters are there? \\
 & & $a^*$: 11,959 \\\hline
\multirow{5}{*}{\texttt{HowManyLonger}} & \multirow{5}{4.0cm}{Asking about the longer distance in questions comparing two distance measures} & $q$: How many yards \textbf{longer} was Rian Lindell's longest field goal \textbf{than his shortest}? \\
 & & $a$: 6 \\
 & & $q^*$: How many yards was Rian Lindell's longest field goal? \\
 & & $a^*$: 28 \\\hline
\multirow{5}{*}{\texttt{HowManyAfter}} & \multirow{5}{4.0cm}{Asking about the later event in questions about time difference of two events} & $q$: \textbf{How many years after} the Treaty of Karlowitz was signed did the Ottomans reclaim the Morea? \\
 & & $a$: 16 \\
 & & $q^*$: \textbf{When} did the Ottomans reclaim the Morea? \\
 & & $a^*$: 1715 \\\hline
 
\multicolumn{3}{c}{\bf Modifying Augmentators} \\ \hline
\multirow{6}{*}{\texttt{CompAntonym}} & \multirow{6}{4.0cm}{Replacing the comparative with its antonym in comparison questions} & $q$: Which was \textbf{higher}, the homeowner vacancy rate or rental vacancy rate? \\
 & & $a$: rental vacancy rate \\
 & & $q^*$: Which was \textbf{lower}, the homeowner vacancy rate or rental vacancy rate? \\
 & & $a^*$: the homeowner vacancy rate \\\hline
\multirow{5}{*}{\texttt{CompRatio}} & \multirow{5}{4.0cm}{Swapping the ratio of numbers correlated to compared objects in comparison questions} & $q$: Which group in Bahrain is larger: Indians or Bangladeshis? \\
 & & $p$: ...roughly 290,000 Indians, \textbf{125,000} Bangladeshis,... \\
 & & $a$: Indians \\
 & & $p^*$: ...roughly 290,000 Indians, \textbf{455,000} Bangladeshis,... \\
 & & $a^*$: Bangladeshis \\\hline
\multirow{4}{*}{\texttt{ComplPercent}} & \multirow{4}{4.0cm}{Asking about the complementary group in percentage questions} & $q$: How many percent of people \textbf{were not} African American? \\
 & & $a$: 98.97 \\
 & & $q^*$: How many percent of people \textbf{were} African American? \\
 & & $a^*$: 1.03 \\\hline
\multirow{5}{*}{\texttt{HowManyMoreSum}} & \multirow{5}{4.0cm}{Asking about the sum rather than the difference in questions about the difference of two numbers} & $q$: How many \textbf{more} masjids are there \textbf{compared to} Buddhist temples? \\
 & & $a$: 5 \\
 & & $q^*$: How many masjids \textbf{and} Buddhist temples are there? \\
 & & $a^*$: 73 \\\hline
\end{tabular}
\end{center}
\caption{Data augmentators.}
\label{table:data_augmentators}
\end{table*}




